Maximal Objectives in the Multi-armed Bandit with Applications

In several applications of the stochastic multi-armed bandit problem, the traditional objective of maximizing the expected total reward can be inappropriate. In this paper, motivated by certain operational concerns in online platforms, we consider a new objective in the classical setup. Given $K$ arms, instead of maximizing the expected total reward from $T$ pulls (the traditional "sum" objective), we consider the vector of total rewards earned from each of the $K$ arms at the end of $T$ pulls and aim to maximize the expected highest total reward across arms (the "max" objective). For this objective, we show that any policy must incur an instance-dependent asymptotic regret of $\Omega(\log T)$ (with a higher instance-dependent constant compared to the traditional objective) and a worst-case regret of $\Omega(K^{1/3}T^{2/3})$. We then design an adaptive explore-then-commit policy featuring exploration based on appropriately tuned confidence bounds on the mean reward and an adaptive stopping criterion, which adapts to the problem difficulty and achieves these bounds (up to logarithmic factors). We then generalize our algorithmic insights to the problem of maximizing the expected value of the average total reward of the top $m$ arms with the highest total rewards. Our numerical experiments demonstrate the efficacy of our policies compared to several natural alternatives in practical parameter regimes. We discuss applications of these new objectives to the problem of grooming an adequate supply of value-providing market participants (workers/sellers/service providers) in online platforms.

==> gen_Intro.tex <==
\section{Introduction}\label{sec:intro}
The stochastic multi-armed bandit (MAB) problem \citep{lai1985asymptotically, auer2002finite} presents a basic formal framework to study the exploration vs. exploitation tradeoff fundamental to online decision-making in uncertain settings. Given a set of $K$ arms, each of which yields independent and identically distributed (i.i.d.) rewards over successive pulls, the goal is to adaptively choose a sequence of arms to maximize the expected value of the total reward attained at the end of $T$ pulls. The critical assumption here is that the reward distributions of the different arms are a priori unknown. Any good policy must hence, over time, optimize the tradeoff between choosing arms that are known to yield high rewards (exploitation) and choosing arms whose reward distributions are yet relatively unknown (exploration).
Over several years of extensive theoretical and algorithmic analysis, this classical problem is now quite well understood (see \cite{lattimore2018bandit}, \cite{slivkins2019introduction}, and \cite{bubeck2012regret} for a survey).\\

In this paper, we address a new objective in this classical setup. We consider the vector of cumulative rewards that have been earned from the different arms at the end of $T$ pulls, and instead of maximizing the expectation of their {\it sum}, \textcolor{red}{we aim to maximize the expected value of the {\it maximum} (max) of these cumulative rewards across the arms}. This problem is motivated by several practical settings, as we discuss below.\\
\textcolor{red}{INSTEAD, SAY THIS?}\\
We consider the vector of cumulative rewards that have been earned from the different arms at the end of $T$ pulls, and instead of maximizing the expectation of their {\it sum}, we aim to maximize the expected value of some percentile of these cumulative rewards across the arms.\\

\begin{enumerate}[wide, labelwidth=!, labelindent=0pt]
	\item {\bf Training workers in online labor platforms.} An important operational objective of online labor platforms is to develop and maintain a reliable pool of high-quality workers to satisfy the demand for jobs. This is a challenging problem since, a) workers continuously leave the platform and hence new talent must be trained on an ongoing basis, b) the number of ``training'' jobs available to train the incoming talent is limited (for instance, this could result from a limited budget for the incentives offered to the clients for choosing novice workers), and c) the quality of the workers is unknown: some workers are fast learners while some are slow, and efficient allocation of training jobs entails distinguishing between these types. 
%Online labor platforms seek to develop and maintain a reliable pool of high-quality workers in steady-state to satisfy the demand for jobs. This is a challenging problem since, a) workers continuously leave the platform and hence new talent must be tended and trained, and b) the number of ``training'' jobs available to the incoming talent is limited (this could, for instance, be because of a limit on the budget for the discounts offered to the clients for choosing novice workers). 
At the core of this challenging operational question is the following problem. Given a limited number of training jobs, the platform must determine a policy to allocate these jobs to a set of novice workers to maximize some appropriate functional of their terminal skill levels. For a platform that seeks to offer robust service guarantees to its clients, simply maximizing the sum of the terminal skill levels across all workers may not be appropriate. A more appropriate objective is to maximize some $q^{\textup{th}}$ percentile skill level amongst the workers ordered by their terminal skills, where $q$ is determined by the volume of demand for regular jobs: higher the demand for jobs, higher the $q$ needed. Effectively, the skill levels of the lower skilled workers at the end of training do not matter, since there is not enough demand for regular jobs to assign to them anyway. 

To address this problem, we can use the MAB framework: the set of arms is the set of novice workers, the reward of an arm is the random increment in the skill level of the worker after performing a job, and the number of training jobs available is $T$. Assuming that $T$ is not too large, the random increments may be assumed to be i.i.d. over time. The mean of these increments can be interpreted as the unknown learning rate or the {\it trainability} of a worker. Given $K$ workers, the goal is to adaptively allocate the jobs to these workers to \textcolor{red}{maximize the smallest terminal skill level amongst the top $m\leq K$ (where $m\approx qK$) most terminally skilled workers}. \textcolor{red}{Our objective corresponds to the case where $m=1$, and is a significant step towards solving this general problem.}\\
\textcolor{red}{BUT WE WILL CONSIDER THE AVG OF TOP-m, DOES IT REQUIRE UPDATING HERE? - ALSO LOSE THE LAST SENTENCE ABOVE}\\

	\item {\bf Training for external competitions.} Related to the above application, the objective we consider is also relevant to the problem of developing advanced talent within a region for participation in external competitions like Science Olympiads, the Olympic games, etc., with limited training resources. In these settings, only the terminal skill levels of those finally chosen to represent the region matter. The resources spent on others, despite resulting in skill advancement, are effectively wasteful. \textcolor{red}{This feature is not captured by the sum objective, while it is effectively captured by the max objective, particularly in situations where one individual will finally be chosen to represent the region.}\\
	\textcolor{red}{INSTEAD, SAY THIS?}\\
	This feature is not captured by the sum objective, while it is effectively captured by the max objective, which corresponds to $\left( \nicefrac{1}{K} \right)^\textup{th}$ percentile, particularly in situations where one individual will finally be chosen to represent the region.\\
	
	\item {\bf Grooming an ``attractor'' product on e-commerce platforms.} E-commerce platforms typically feature very similar substitutes within a product category. For instance, consider a product like a tablet cover (e.g., for an iPad). Once the utility of a new product of this type becomes established (e.g., the size specifications of a new version of the iPad becomes available), several brands offering close to identical products serving the same purpose proliferate the marketplace. This proliferation is problematic to the platform for two reasons: a) customers are inundated by choices and may unnecessarily delay their purchase decision, thereby increasing the possibility of leaving the platform altogether \citep{settle1974consumer, gourville2005overchoice}, and b) the heterogeneity in the purchase behavior resulting from the lack of a clear choice may complicate the problem of effectively managing inventory and delivery logistics. Given a budget for incentivizing customers to pick different products in the early exploratory phase where the qualities of the different products are being discovered, a natural objective for the platform is to ``groom'' a product to have the highest volume of positive ratings at the end of this phase. This product then becomes a clear choice for the customers. Our objective effectively captures this goal.
\end{enumerate}

\textcolor{red}{more examples for the general $m$ case rather than examples \textit{entirely} focused on $m=1$.}//


A key assumption we make in the paper is that the rewards for all arms are non-negative; this is motivated by training applications where rewards represent skill increments. Under this assumption, in the {\it full-information} setting where the reward distributions of the arms are known, we first show that the optimal policy for the max objective is identical to the one for the sum objective: one always pulls the arm(s) with the highest mean reward(s) (Proposition~\ref{prop_general:main}). This additionally implies that the optimal rewards under the two objectives are identical.  


A standard approach in MAB problems is to design a policy that minimizes {\it regret}, i.e., the quantity of loss relative to the optimal full-information policy for a given objective over time. 
In the classical setting with the sum objective, it is well known that any policy must incur an instance-dependent asymptotic regret of $\Omega(\sum_{i\neq i^*} (\Delta_i\log T)/d_i)$ as $T\rightarrow \infty$ \citep{lai1985asymptotically}. Here, $\Delta_i = \mu^*-\mu_i$, i.e., it is the difference between the highest mean reward $\mu^*$ belonging to the arm $i^*$ and the mean reward $\mu_i$ of arm $i$; and $d_i$ is a quantity that captures an appropriate notion of divergence between the reward distribution of arm $i$ and the ``closest'' distribution within the space of possible distributions having a mean that is at least $\mu^*$. Additionally, it is also well-known that any policy must incur and instance-independent regret of $\Omega(\sqrt{KT})$ in the worst-case over the set of possible bandit instances \citep{auer2002finite}. 

Since the optimal full-information reward is the same under the sum and the max objectives, and since the maximum of a set of non-negative numbers is always at most the sum of the numbers, any lower bound on the regret for the sum objective implies the same lower bound on the max objective. However, a key feature of the max objective is that the rewards earned from arms that do not eventually turn out to be the one \textcolor{red}{yielding the highest cumulative reward are effectively a waste.} SAY  However, a key feature of the max objective is that the rewards earned from arms that do not eventually turn out to be the ones yielding the highest cumulative rewards are effectively a waste. 

\textcolor{red}{This is for $m=1$. Put general $m$ results here and push this part after it.}
Owing to this feature, we show that any policy must incur a {\it higher} instance-dependent regret of $\Omega(\sum_{i\neq i^*} (\mu^*\log T)/{d_i})$ in this case (Theorem~\ref{thm:asymplwb}). Moreover, we show that an instance-independent regret of $\Omega(K^{1/3}T^{2/3})$ is inevitable in the worst-case (Theorem~\ref{thm:lb}). Both these results rely on novel arguments that are a significant departure from those involved in proving the corresponding lower bounds for the sum objective.

Attaining these lower bounds requires algorithmic innovation. For the sum objective, well-performing policies are typically based on the principle of optimism in the face of uncertainty. A popular policy-class is the Upper Confidence Bound (UCB) class of policies \citep{agrawal1995sample,auer2002finite,auer2010ucb}, in which a confidence interval is maintained for the mean reward of each arm, and at each time, the arm with the highest upper confidence bound is chosen. For a standard tuning of these intervals, this policy -- termed UCB1 in literature due to \citep{auer2002finite} -- guarantees an instance-dependent asymptotic regret of $\textup{O}(\log T)$ and a regret of $\textup{O}(\sqrt{KT\log T})$ in the worst case. With a more refined tuning, $\textup{O}(\sqrt{KT})$ can be achieved \citep{audibertminimax, lattimore2018refining}. 

\textcolor{red}{This is for $m=1$, need to update this for general $m$.} For our max objective, directly using one of the above UCB policies can prove to be disastrous.
To see this, suppose that all $K$ arms have equal deterministic rewards. Then, UCB1 will pull each of the arms in a round-robin fashion until a total of $T$ pulls, resulting in the highest terminal cumulative reward of $\textup{O}(T/K)$; whereas, a reward of $\Theta(T)$ is feasible by simply committing to an arbitrary arm from the start. 
This results in a $\Omega(T)$ regret in the worst case. Introducing randomness in the rewards doesn't change this observation: the result of a numerical experiment shown in Figure~\ref{fig:regret} suggests a $\Omega(T)$ regret on using UCB1 for a two-armed bandit problem with both arms having Bernoulli rewards with mean $0.5$. 


\textcolor{red}{These two paragraphs are for $m=1$}\\
This observation suggests that any good policy must, at some point, stop exploring and permanently commit to \textcolor{red}{a single arm}. A natural candidate is the basic explore-then-commit (ETC) strategy, which uniformly explores all arms until some time that is fixed in advance, and then commits to the empirically best arm \citep{lattimore2018bandit, slivkins2019introduction}. When each arm is chosen $(T/K)^{2/3}$ times in the exploration phase, this strategy can be shown to achieve a regret of $\textup{O}(K^{1/3}T^{2/3}\sqrt{\log K})$ relative to the sum objective \citep{slivkins2019introduction}. It is easy to argue that it achieves the same regret relative to the max objective. However, this policy is excessively optimized for the worst case where the means of all the arms are within $(K/T)^{1/3}$ of each other. When the arms are easier to distinguish, this policy's performance is quite poor due to excessive exploration. For example, consider a two armed bandit problem with Bernoulli rewards and means $(0.5, 0.5+\Delta)$, where $\Delta>0$. For this fixed instance, ETC will pull both arms $\Omega(T^{2/3})$ times and hence incur a regret of $\Omega(T^{2/3})$ relative to our max objective. However, it is well known that UCB1 will not pull the suboptimal arm more than $\textup{O}(\log T/\Delta^2)$ times with high probability \citep{auer2002finite} and hence for this instance, UCB1 will incur an instance-dependent regret of only $\textup{O}(\log T)$, which could be much smaller if $\Delta$ is large. Thus, although the worst case regret of UCB1 is $\Omega(T)$ due to perpetual exploration, for a fixed bandit instance, its asymptotic performance is significantly better than ETC. This observation motivates us to seek a practical policy with a graceful dependence of performance on the difficulty of the bandit instance, and which will achieve both: the worst-case bound of ETC and the instance-dependent asymptotic bound of $\textup{O}(\log T)$.

We propose a new policy with an explore-then-commit structure, in which appropriately defined confidence bounds on the means of the arms are utilized to guide exploration, as well as to decide when to stop exploring. We call this policy Adaptive Explore-then-Commit (ADA-ETC). 
%Compared to the classical UCB1 way of defining the confidence intervals, our policy's confidence bounds are finely tuned to eliminate wasteful exploration and encourage stopping early if appropriate. %We derive rigorous instance-dependent as well as worst-case bounds on the regret guaranteed by this policy. 
We show that ADA-ETC adapts to the problem difficulty by exploring less if appropriate, while attaining the same regret guarantee of $\textup{O}(K^{1/3}T^{2/3}\sqrt{\log K})$ attained by vanilla ETC in the worst case (Theorem~\ref{thm_stopping}). %Whether the $\sqrt{\log K}$ factor can be eliminated as well remains an open question. 
In particular, ADA-ETC guarantees an instance-dependent asymptotic regret of $\textup{O}(\log T)$ as $T\rightarrow\infty$, matching our instance-dependent lower bound upto a constant factor. Finally, our numerical experiments demonstrate that ADA-ETC results in significant improvements over the performance of vanilla ETC in easier settings, while never performing worse in difficult ones, thus corroborating our theoretical results. Our numerical results also demonstrate that naive ways of introducing adaptive exploration based on upper confidence bounds, e.g., simply using the upper confidence bounds of UCB1, may lead to no improvement over vanilla ETC for practical values of $T$ and $K$.

\subsection{Related literature}
To the best of our knowledge, the objective we consider in this paper has not been studied before. We nevertheless note that buried in our objective is the goal of quickly identifying the arm with approximately the highest mean reward so that a substantial amount of time can be spent earning rewards from that arm (e.g., ``training'' a worker). This goal is related to the {\it pure exploration} problem in multi-armed bandits. Several variants of this problem have been studied, where the goal of the decision-maker is to either minimize the probability of misidentification of the optimal arm given a fixed budget of pulls \citep{audibert2010best, kaufmann2016complexity, carpentier2016tight}; or minimize the expected number of pulls to attain a fixed probability of misidentification, possibly within an approximation error \citep{even2002pac, mannor2004sample, even2006action, karnin2013almost, vaidhiyan2017learning, jamieson2014lil, kaufmann2016complexity}; or to minimize the expected suboptimality (called ``simple regret'') of a recommended arm after a fixed budget of pulls \citep{bubeck2009pure, bubeck2011pure, carpentier2015simple}. Extensions to settings where multiple good arms are needed to be identified have also been considered \citep{bubeck2013multiple, kalyanakrishnan2012pac, zhou2014optimal, kaufmann2013information}. The critical difference from these approaches is that in our scenario, the budget of $T$ pulls must not only be spent on identifying an approximately optimal arm but also on earning rewards on that arm. Hence any choice of apportionment of the budget to the identification problem, or a choice for a target for the approximation error or probability of misidentification within a candidate policy, is a priori unclear and must arise {\it endogenously} from our primary objective. 

The fact that focusing on one arm in the long-run is prudent for our objective makes it seem related to the line of work on bandits with switching costs, where there is a cost incurred for switching from one arm to another \citep{cesa2013online, dekel2014bandits}. Another related line of work is on {\it batched} bandits, which imposes a constraint that the policy must split the arm pulls into a small number of batches \citep{perchet2016batched, gao2019batched}. However, we note that our objective does not simply amount to keeping the number of switches or batches low; it also matters how ``spread apart'' the switches are. To enforce this point, we note that the algorithm of \cite{cesa2013online}, which restricts the number of switches/batches to $\textup{O}(\log \log T)$ while attaining $\tilde{\textup{O}}(\sqrt{T})$ regret for the sum objective, incurs a worst-case regret of $\Theta(T)$ for our max objective: Figure~\ref{fig:regret} shows this for $K=2$ arms with Bernoulli(0.5) rewards. 

\begin{figure}[h]
	\centering
	\includegraphics[width=0.4\textwidth]{regret}
	\caption{Expected regret for the max objective under UCB1 and the algorithm of \cite{cesa2013online}, referred to here as {\it Switch}, for $K=2$ arms, each with Bernoulli$(0.5)$ rewards.}\label{fig:regret}
\end{figure}

==> gen_lower-bound.tex <==
\subsection{Lower Bound}\label{sec:lb_general}
\begin{theorem}\label{thm_general:lb}
	Suppose that $m \leq K/2$ and $K < T$. Then, $\PPSR^*_T \geq  \Omega\left(\frac{(K-m)^{1/3} T^{2/3}}{m^{4/3}}\right).$
\end{theorem}
The proof is presented in Section~\ref{apx_general:lb} in the Appendix.

==> gen_numerics_backup.tex <==
\subsection{$\boldsymbol{m}$-ADA-ETC} \label{sec:numerics_general}
%{\bf Benchmark Algorithms.} 
We compare the performance of $m\textup{-ADA-ETC}$ with four algorithms described in Table~\ref{algorithms_m}. %UCB1 never stops exploring and pulls the arm with the highest upper confidence bound at each time step, while 
$m\textup{-ETC}$ pulls arms in a round-robin fashion and commits to the $m$ arms with the highest empirical means after each arm has been pulled $\tau$ times. As before, $m\textup{-NADA-ETC}$ and $m\textup{-UCB1-s}$ have the same algorithmic structure as $m\textup{-ADA-ETC}$: they explore based on upper confidence bounds and commit if the lower confidence bound of all arms rise above the upper confidence bounds of all other arms. They differ from $m\textup{-ADA-ETC}$ in how the upper and lower confidence bounds are defined. This time we exclude $m\textup{-UCB1-s}$ from our figures for brevity since, as before, its performance is identical to that of $m\textup{-NADA-ETC}$ for the parameter sets we focus on.

\begin{table}[h]
	\caption{Benchmark Algorithms}
	\label{algorithms_m}
	\centering\scriptsize{
		\begin{tabular}{lll}
			\toprule
			\vspace{-0.1cm}\\
			\multirow{2}{*}{$m\textup{-ADA-ETC}$}&$\ucb^i_n=$ $\bar{\mu}_n^i + \sqrt{\frac{4}{n}\log\left(\frac{T}{(K-m)n^{3/2}}\right)}\mathbbm{1}_{\left\{ n< \tau \right\}}$\\\vspace{0.15cm}&$\lcb^i_n=$ $\bar{\mu}_n^i - \bar{\mu}_n^i\mathbbm{1}_{\{n< \tau\}}$\\
			\multirow{2}{*}{$m\textup{-ETC}$}&$\ucb^i_n=$ $*$\\\vspace{0.15cm}&$\lcb^i_n=$ $*$\\
			\multirow{2}{*}{$m\textup{-NADA-ETC}$}&$\ucb^i_n=$ $\bar{\mu}_n^i + \sqrt{\frac{4}{n}\log\left(T\right)}\mathbbm{1}_{\left\{ n< \tau \right\}}$\\\vspace{0.15cm}&$\lcb^i_n=$ $\bar{\mu}_n^i - \bar{\mu}_n^i\mathbbm{1}_{\{n< \tau\}}$\\
			\multirow{2}{*}{$m\textup{-UCB1-s}$}&$\ucb^i_n=$ $\bar{\mu}_n^i + \sqrt{\frac{4}{n}\log\left(T\right)}\mathbbm{1}_{\left\{ n< \tau \right\}}$ \\&$\lcb^i_n=$ $\bar{\mu}_n^i - \sqrt{\frac{4}{n}\log\left(T\right)}\mathbbm{1}_{\left\{ n< \tau \right\}}$\\
			\multirow{2}{*}{RADA-ETC}&$\ucb^i_n=$ $\bar{\mu}_n^i + \sqrt{\frac{4}{n}\log\left(\frac{T}{Kn^{3/2}}\right)}\mathbbm{1}_{\left\{ n< \tau \right\}}$\\\vspace{0.15cm}&$\lcb^i_n=$ $\bar{\mu}_n^i - \bar{\mu}_n^i\mathbbm{1}_{\{n< \tau\}}$\\
			\vspace{-0.1cm}\\
			\bottomrule
		\end{tabular}
	}
\end{table}

Additionally, we introduce a natural benchmark that utilizes ADA-ETC, which we call randomized ADA-ETC (RADA-ETC).
RADA-ETC randomly groups $K$ arms into $m$ subsets of size $K/m$ and runs ADA-ETC (until the end of Explore phase) for each subset with a budget of $T/m$ and returns one arm from each subset. Those arms are then pulled until the total number of remaining pulls allows. These definitions are presented in Table~\ref{algorithms_m}.

%\vspace{0.1cm}


\noindent{\bf Instances.} We let $\nu_i \sim \textup{Bernoulli}(\mu_i)$, where $\mu_i$ is uniformly sampled from $[\alpha, 1-\alpha]$ for each arm in each instance. We sample two sets of instances, each of size $250$, with $\alpha \in\{0, 0.4\}$. The regret for an algorithm for each instance is averaged over $100$ runs to estimate the expected regret. 
We vary $m \in \{2, 5, 10 \}$, $K \in \{4, 20\}$ and $T \in \{100, 200, 300, 400, 500\}$. The average regret over the $250$ instances under different algorithms and settings is presented in Figures~\ref{fig:experiments_m1} and~\ref{fig:experiments_m2}.

\begin{figure}[h]
	\centering
	\hspace{1cm}
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K4_m2_alpha0NEW.eps}
		\caption{$m=2$, $K=4$, $\alpha = 0$}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K20_m10_alpha0NEW.eps}
		\caption{$m=10$, $K=20$, $\alpha = 0$}
	\end{subfigure} \hspace{1cm}
	%
		
	\vspace{0.3cm}
	\hspace{1cm}
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K4_m2_alpha0_4NEW.eps}
		\caption{$m=2$, $K=4$, $\alpha = 0.4$}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K20_m10_alpha0_4NEW.eps}
		\caption{$m=10$, $K=20$, $\alpha = 0.4$}
	\end{subfigure} \hspace{1cm}
	%
	\caption{Performance comparison of $\boldsymbol{m}\textup{-ADA-ETC}$ for varying values of $T$.} \label{fig:experiments_m1}
\end{figure}

%\begin{figure}[h]
%	\hspace{1.25cm}
%	\subfloat[$m=2$, $K=4$, $\alpha = 0$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K4_m2_alpha0NEW.eps}} \hfill
%	\subfloat[$m=10$, $K=20$, $\alpha = 0$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K20_m10_alpha0NEW.eps}} \hspace{1.25cm}
%	\caption{Performance comparison of $\boldsymbol{m}\textup{-ADA-ETC}$ for varying values of $T$. Note that $\boldsymbol{m}\textup{-ETC}$ is outperforming RADA-ETC here.\label{fig:experiments_m11}}
%\end{figure}
%\begin{figure}[h]
%	\hspace{1.25cm}
%	\subfloat[$m=2$, $K=4$, $\alpha = 0.4$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K4_m2_alpha0_4NEW.eps}} \hfill
%	\subfloat[$m=10$, $K=20$, $\alpha = 0.4$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K20_m10_alpha0_4NEW.eps}} \hspace{1.25cm}
%	\caption{Performance comparison of $\boldsymbol{m}\textup{-ADA-ETC}$ for varying values of $T$. \label{fig:experiments_m12}}
%\end{figure}

\noindent{\bf Discussion.} While $m\textup{-ADA-ETC}$ shows the best performance uniformly across almost all settings, $m\textup{-ETC}$ or RADA-ETC perform almost as good in some settings.


Similar to the $m=1$ case, $m\textup{-ETC}$ is expected to perform as good as $m\textup{-ADA-ETC}$ when we either have (a) $\alpha = 0.4$, that is, the arms are expected to be close to each other and so that adaptivity in exploring is not as beneficial, or (b) $T/(K-m)$ is small, so that $\tau$ is small and is likely to be exhausted under $m\textup{-ADA-ETC}$. %We observe this trend in Figures~\ref{fig:experiments_m1} (c)-(d) and Figures~\ref{fig:experiments_m2} (c)-(d), when compared to Figures~\ref{fig:experiments_m1} (a)-(b) and Figures~\ref{fig:experiments_m2} (a)-(b).

We find a mild anomaly to this trend in Figures~\ref{fig:experiments_m2} (c)-(d). In this case, we notice that even when $\alpha = 0.4$, and $\tau$ in (c) is smaller than $\tau$ in (d), the performance of $m\textup{-ETC}$ is significantly worse than $m\textup{-ADA-ETC}$ in (c) compared to (d). This can be explained by the fact that $K-m$ is larger for (c) than for (d), and thus the confidence bounds of  $m\textup{-ADA-ETC}$ are relatively smaller in (c) compared to those in (d). This encourages an early stop to the exploration compared to $m\textup{-ETC}$ despite the smaller $\tau$. 
%Take Figures~\ref{fig:experiments_m1} (c)-(d) first: $\tau$ in (d) is smaller than $\tau$ in (c), and $m\textup{-ADA-ETC}$ outperforms $m\textup{-ETC}$ in (c). But, in Figures~\ref{fig:experiments_m2} (c)-(d), we see that $\tau$ in (c) is smaller than $\tau$ in (d), and yet $m\textup{-ADA-ETC}$ outperforms $m\textup{-ETC}$ in (c). 
%This is due to the adaptive nature of upper confidence bounds defined in $m\textup{-ADA-ETC}$: as $K-m$ becomes larger, although the number of pulls per arm during the Explore phase gets smaller, the upper confidence bounds get tighter and hence $m\textup{-ADA-ETC}$ may stop exploring earlier, even when the arms are expected to be close to each other.


\begin{figure}[h]
	\centering
	\hspace{1cm}
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K20_m2_alpha0NEW.eps}
		\caption{$m=2$, $K=20$, $\alpha = 0$}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K20_m5_alpha0NEW.eps}
		\caption{$m=5$, $K=20$, $\alpha = 0$}
	\end{subfigure} \hspace{1cm}
	%
	
	\vspace{0.3cm}
	\hspace{1cm}
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K20_m2_alpha0_4NEW.eps}
		\caption{$m=2$, $K=20$, $\alpha = 0.4$}
	\end{subfigure}%
	\hfill
	\begin{subfigure}{0.4\textwidth}
		\centering
		\includegraphics[width=\textwidth]{100sim_250armdist_4bench_K20_m5_alpha0_4NEW.eps}
		\caption{$m=5$, $K=20$, $\alpha = 0.4$}
	\end{subfigure} \hspace{1cm}
	%
	\caption{Performance comparison of $\boldsymbol{m}\textup{-ADA-ETC}$ for varying values of $T$.} \label{fig:experiments_m2}
\end{figure}

%\begin{figure}[h]
%	\hspace{1.25cm}
%	\subfloat[$m=2$, $K=20$, $\alpha = 0$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K20_m2_alpha0NEW.eps}} \hfill
%	\subfloat[$m=5$, $K=20$, $\alpha = 0$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K20_m5_alpha0NEW.eps}} \hspace{1.25cm}
%	\caption{Performance comparison of $\boldsymbol{m}\textup{-ADA-ETC}$ for varying values of $T$. 
%		\label{fig:experiments_m21}}
%\end{figure}

%\begin{figure}[h]
%	\hspace{1.25cm}
%	\subfloat[$m=2$, $K=20$, $\alpha = 0.4$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K20_m2_alpha0_4NEW.eps}} \hfill
%	\subfloat[$m=5$, $K=20$, $\alpha = 0.4$ ]{\includegraphics[width = 0.35\textwidth]{100sim_250armdist_4bench_K20_m5_alpha0_4NEW.eps}} \hspace{1.25cm}
%	\caption{Performance comparison of $\boldsymbol{m}\textup{-ADA-ETC}$ for varying values of $T$. The performance of RADA-ETC is on par with $\boldsymbol{m}\textup{-ADA-ETC}$.
%		\label{fig:experiments_m22}}
%\end{figure}



%Despite this similarity, looking at Figures~\ref{fig:experiments_m1} (c)-(d) and Figures~\ref{fig:experiments_m2} (c)-(d), we notice that even when $\alpha = 0.4$, the performance of $m\textup{-ETC}$ can be worse than $m\textup{-ADA-ETC}$.
%Take Figures~\ref{fig:experiments_m1} (c)-(d) first: $\tau$ in (d) is smaller than $\tau$ in (c), and $m\textup{-ADA-ETC}$ outperforms $m\textup{-ETC}$ in (c). But, in Figures~\ref{fig:experiments_m2} (c)-(d), we see that $\tau$ in (c) is smaller than $\tau$ in (d), and yet $m\textup{-ADA-ETC}$ outperforms $m\textup{-ETC}$ in (c). 
%This is due to the adaptive nature of upper confidence bounds defined in $m\textup{-ADA-ETC}$: as $K-m$ becomes larger, although the number of pulls per arm during the Explore phase gets smaller, the upper confidence bounds get tighter and hence $m\textup{-ADA-ETC}$ may stop exploring earlier, even when the arms are expected to be close to each other.


%	Although looking at Figures~\ref{fig:experiments_m1} (c)-(d) and Figures~\ref{fig:experiments_m2} (c)-(d), we notice some discrepancies, e.g., $\alpha = 0.4$ alone is not sufficient for $m\textup{-ETC}$ to perform similar to $m\textup{-ADA-ETC}$. Take Figures~\ref{fig:experiments_m1} (c)-(d): $\tau$ for (c) is larger than $\tau$ for (d), and $m\textup{-ADA-ETC}$ outperforms $m\textup{-ETC}$ in (c). But, in Figures~\ref{fig:experiments_m2} (c)-(d), we see that $\tau$ for (c) is smaller than $\tau$ for (d), yet $m\textup{-ADA-ETC}$ still outperforms $m\textup{-ETC}$ in (c). This suggests that, even though the number of pulls per arm during the Explore phase gets smaller as $K/m$ grows, the fact that a smaller number of arms ($2$ versus $5$ in Figures~\ref{fig:experiments_m2} (c)-(d)) will be pulled in the Commit phase makes a difference (total pulls per arm in case of $m=2$ is larger than that of $m=5$). Hence, $m\textup{-ADA-ETC}$ entering the Commit phase earlier in some cases is worth more as $K/m$ grows.

We then look at the performance of RADA-ETC. The only scenarios where its performance comes close to that of $m$-ADA-ETC are those in Figures~\ref{fig:experiments_m2} (c)-(d). Here, since the size of the random subsets $(K/m)$ is relatively large and arm means are close to each other, the probability of the best arm in a random subset being significantly suboptimal is lower.   

%First, we observe that although $\alpha = 0$ in Figures~\ref{fig:experiments_m1} (a)-(b) and Figures~\ref{fig:experiments_m2} (a)-(b), error bars are significantly narrower in Figure~\ref{fig:experiments_m2} (a). Since $m=2$ in Figure~\ref{fig:experiments_m2} (a), there are two subsets to be randomly generated and the probability of the two optimal arms ending up in the same subset is high. But since $K/m$ is also higher, compared to the other parameter sets, the probability of two ``good'' arms ending up in the same subset across all random subsets is lower, and hence the variation in average rewards is smaller.

% observe that RADA-ETC outperforming $m\textup{-ETC}$ does not solely depend on the choice of $\alpha$ value. $m\textup{-ETC}$ outperforms RADA-ETC when $\alpha = 0$, except for the setting in Figure~\ref{fig:experiments_m2} (a). On the other hand, RADA-ETC outperforms $m\textup{-ETC}$ when $\alpha = 0.4$, except for the setting in Figure~\ref{fig:experiments_m1} (d). Former is due to the above observation: Since $K/m$ is higher and therefore the probability of two ``good'' arms ending up in the same subset across all random subsets is lower, RADA-ETC enjoys the advantage of ADA-ETC in quickly identifying good arms, outperforming $m\textup{-ETC}$ in Figure~\ref{fig:experiments_m2} (a). Latter is due to the specific parameter setting: There are $10$ different subsets with $2$ arms each and both arms in all subsets are expected to be close to each other. Hence, all the exploration budget is likely to be used for all subsets. But there is still room for misidentification as only one arm from each subset can be selected to be included in Commit phase. $m\textup{-ETC}$ does not have this constraint and therefore outperforms RADA-ETC.

%{\color{blue} 
%	We can then look at the performance of RADA-ETC.
%	We make two observations: (1) Although $\alpha = 0$ in Figures~\ref{fig:experiments_m1} (a)-(b) and Figures~\ref{fig:experiments_m2} (a)-(b), error bars are significantly narrower in Figure~\ref{fig:experiments_m2} (a). This is because $K/m$ is higher for the parameters in Figure~\ref{fig:experiments_m2} (a), implying that the probability of two same ``good'' arms ending up in different subsets is higher, 
%	{\color{red} (VK:wouldn't this probability decrease?)-- E:Yes, not worded same as what i had in mind, needs fix, can say $<$since the subsets are larger, the probability of ADA-ETC selecting the same two arms from both subsets in different random groupings is higher$>$}  and hence the variation in average rewards is smaller. 
%	(2) RADA-ETC outperforming $m\textup{-ETC}$ does not solely depend on $\alpha$. $m\textup{-ETC}$ outperforms RADA-ETC when $\alpha = 0$, except for the setting in Figure~\ref{fig:experiments_m2} (a). Similarly, RADA-ETC outperforms $m\textup{-ETC}$ when $\alpha = 0.4$, except for the setting in Figure~\ref{fig:experiments_m1} (d). 
%	Former is due to the first observation: {\color{red} since the probability of two optimal arms ending up in different subsets is a lot higher}, RADA-ETC enjoys performance guarantee of $m\textup{-ADA-ETC}$ and outperforms $m\textup{-ETC}$ in Figure~\ref{fig:experiments_m2} (a). Latter is due to the specific parameter setting: $10$ different subsets with $2$ arms each implies that the probability of grouping at least two ``good'' arms in the same subset is high, and hence the regret is slightly higher for RADA-ETC {\color{red} (VK:wouldn't the probability of two good arms falling in the same subset be lower if there are more subsets?)-- i think the problem here is all the exploration budget is used in RADA-ETC and still there is room for misidentification because of the subsets and hard selection rules - $m\textup{-ADA-ETC}$ is okay since it doesn't have the same problem of a hard selection, same for ETC} .
%}


And finally, as in the $m=1$ case, $m\textup{-NADA-ETC}$ is not a suitable alternative to $m\textup{-ADA-ETC}$, thus illustrating the gains from the tuning of the confidence bounds under $m\textup{-ADA-ETC}$.
